From FATS to feets: Further improvements to an astronomical feature extraction tool based on machine learning

Machine learning algorithms are highly useful for the classification of time series data in astronomy in this era of peta-scale public survey data releases. These methods can facilitate the discovery of new unknown events in most astrophysical areas, as well as improving the analysis of samples of known phenomena. Machine learning algorithms use features extracted from collected data as input predictive variables. A public tool called Feature Analysis for Time Series (FATS) has proved an excellent workhorse for feature extraction, particularly light curve classification for variable objects. In this study, we present a major improvement to FATS, which corrects inconvenient design choices, minor details, and documentation for the re-engineering process. This improvement comprises a new Python package called "feets", which is important for future code-refactoring for astronomical software tools.

==> stylecheck.tex <==
\begin{minted}[]{bash}
$ git rev-parse HEAD
ddedb00b527cea2e2ccd760a460bea23029a8dce

$ flake8 --version
3.5.0 (mccabe: 0.6.1, pycodestyle: 2.3.1, pyflakes: 1.6.0) CPython 2.7.6 on Linux

$ flake8 setup.py FATS/ --statistics --count | tail -n 36
6     E101 indentation contains mixed spaces and tabs
63    E111 indentation is not a multiple of four
14    E114 indentation is not a multiple of four (comment)
1     E127 continuation line over-indented for visual indent
7     E201 whitespace after '('
6     E202 whitespace before ')'
7     E203 whitespace before ','
9     E221 multiple spaces before operator
1     E222 multiple spaces after operator
33    E225 missing whitespace around operator
50    E231 missing whitespace after ','
6     E251 unexpected spaces around keyword / parameter equals
1     E262 inline comment should start with '# '
18    E265 block comment should start with '# '
1     E301 expected 1 blank line, found 0
24    E302 expected 2 blank lines, found 0
7     E303 too many blank lines (2)
1     E305 expected 2 blank lines after class or function definition, found 1
2     E401 multiple imports on one line
118   E501 line too long (81 > 79 characters)
1     E701 multiple statements on one line (colon)
2     E711 comparison to None should be 'if cond is None:'
3     E712 comparison to True should be 'if cond is True:' or 'if cond:'
2     E713 test for membership should be 'not in'
34    E722 do not use bare except'
35    F401 'sys' imported but unused
3     F403 'from FeatureFunctionLib import *' used; unable to detect undefined names
10    F405 'zeros' may be undefined, or defined from star imports: numpy, numpy.fft
11    F811 redefinition of unused 'time' from line 3
4     F841 local variable 'time' is assigned to but never used
145   W191 indentation contains tabs
175   W291 trailing whitespace
2     W292 no newline at end of file
41    W293 blank line contains whitespace
3     W391 blank line at end of file
846

$ sloccount --version
2.26

$ sloccount FATS/ setup.py 
Creating filelist for FATS
Have a non-directory at the top, so creating directory top_dir
Adding /home/jbcabral/projects/FATS/src/setup.py to top_dir
Categorizing files.
Finding a working MD5 command....
Found a working MD5 command.
Computing results.

SLOC	Directory	SLOC-by-Language (Sorted)
1334    FATS            python=1334
34      top_dir         python=34

Totals grouped by language (dominant language first):
python:        1368 (100.00%)

Total Physical Source Lines of Code (SLOC)                = 1,368
Development Effort Estimate, Person-Years (Person-Months) = 0.28 (3.34)
 (Basic COCOMO model, Person-Months = 2.4 * (KSLOC**1.05))
Schedule Estimate, Years (Months)                         = 0.33 (3.95)
 (Basic COCOMO model, Months = 2.5 * (person-months**0.38))
Estimated Average Number of Developers (Effort/Schedule)  = 0.84
Total Estimated Cost to Develop                           = $ 37,543
 (average salary = $56,286/year, overhead = 2.40).
SLOCCount, Copyright (C) 2001-2004 David A. Wheeler
SLOCCount is Open Source Software/Free Software, licensed under the GNU GPL.
SLOCCount comes with ABSOLUTELY NO WARRANTY, and you are welcome to
redistribute it under certain conditions as specified by the GNU GPL license;
see the documentation for details.
Please credit this data as "generated using David A. Wheeler's 'SLOCCount'."
\end{minted}

